Powerful genome-wide design and robust statistical inference in two-sample summary-data Mendelian randomization

Two-sample summary-data Mendelian randomization (MR) has become a popular research design to estimate the causal effect of risk exposures. With the sample size of GWAS continuing to increase, it is now possible to utilize genetic instruments that are only weakly associated with the exposure. To maximize the statistical power of MR, we propose a genome-wide design where more than a thousand genetic instruments are used. For the statistical analysis, we use an empirical partially Bayes approach where instruments are weighted according to their strength, thus weak instruments bring less variation to the estimator. The estimator is highly efficient with many weak genetic instruments and is robust to balanced and/or sparse pleiotropy. We apply our method to estimate the causal effect of body mass index (BMI) and major blood lipids on cardiovascular disease outcomes and obtain substantially shorter confidence intervals. Some new and statistically significant findings are: the estimated causal odds ratio of BMI on ischemic stroke is 1.19 (95% CI: 1.07--1.32, p-value < 0.001); the estimated causal odds ratio of high-density lipoprotein cholesterol (HDL-C) on coronary artery disease (CAD) is 0.78 (95% CI 0.73--0.84, p-value < 0.001). However, the estimated effect of HDL-C becomes substantially smaller and statistically non-significant when we only use the strong instruments. By employing a genome-wide design and robust statistical methods, the statistical power of MR studies can be greatly improved. Our empirical results suggest that, even though the relationship between HDL-C and CAD appears to be highly heterogeneous, it may be too soon to completely dismiss the HDL hypothesis.

==> introduction.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> result2.tex <==
%% LDL
\begin{table} \footnotesize \centering
% \begin{subtable}[t]{\textwidth} \centering
% \begin{tabular}{lcccccc}
% \hline
%  & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
% \hline
% \# SNPs  & \multicolumn{2}{c}{1153} & \multicolumn{2}{c}{36} & \multicolumn{2}{c}{1117} \\
% $p_1$  & \multicolumn{2}{c}{0.92} & \multicolumn{2}{c}{0.99} & \multicolumn{2}{c}{0.9} \\
% $\sigma_1$  & \multicolumn{2}{c}{0.51} & \multicolumn{2}{c}{9.62} & \multicolumn{2}{c}{0.41} \\
% $\sigma_2$  & \multicolumn{2}{c}{6.43} & \multicolumn{2}{c}{9.62} & \multicolumn{2}{c}{2.44} \\
% Egger  & \multicolumn{2}{c}{0.302 (0.042)} & \multicolumn{2}{c}{0.387 (0.118)} & \multicolumn{2}{c}{-0.012 (0.079)} \\
% Wtd.\ Med.  & \multicolumn{2}{c}{0.21 (0.061)} & \multicolumn{2}{c}{0.255 (0.066)} & \multicolumn{2}{c}{0.024 (0.086)} \\
% \hline %  &  &  &  &  &  &  \\
%   & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
% $\tau^2 = 0$, $\rho_{l_2}$  & 0.331 (0.042) & 0.353 (0.038) & 0.389 (0.039) & 0.389 (0.039) & 0.002 (0.17) & 0.089 (0.124) \\
% $\tau^2 = 0$, $\rho_H$  & 0.332 (0.042) & 0.346 (0.038) & 0.411 (0.04) & 0.411 (0.04) & 0.092 (0.146) & 0.13 (0.112) \\
% $\tau^2 \ne 0$, $\rho_{l_2}$  & 0.3 (0.045) & 0.339 (0.042) & 0.389 (0.057) & 0.389 (0.057) & -0.007 (0.126) & 0.07 (0.111) \\
% $\tau^2 \ne 0$, $\rho_H$  & 0.299 (0.045) & 0.328 (0.042) & 0.381 (0.056) & 0.381 (0.056) & 0.052 (0.129) & 0.106 (0.111) \\
% \hline
% \end{tabular}
% \caption{Using unrestricted SNPs.}
% \label{tab:ldl-1}
% \end{subtable}\vspace{6pt}
% \begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1120} & \multicolumn{2}{c}{27} & \multicolumn{2}{c}{1093} \\
$p_1$  & \multicolumn{2}{c}{0.92} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.91} \\
$\sigma_1$  & \multicolumn{2}{c}{0.52} & \multicolumn{2}{c}{7.96} & \multicolumn{2}{c}{0.46} \\
$\sigma_2$  & \multicolumn{2}{c}{5.01} & \multicolumn{2}{c}{7.96} & \multicolumn{2}{c}{2.61} \\
Egger  & \multicolumn{2}{c}{0.368 (0.053)} & \multicolumn{2}{c}{0.892 (0.134)} & \multicolumn{2}{c}{0.057 (0.08)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.534 (0.071)} & \multicolumn{2}{c}{0.552 (0.075)} & \multicolumn{2}{c}{0.166 (0.094)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & 0.448 (0.06) & 0.484 (0.05) & 0.528 (0.055) & 0.528 (0.055) & 0.204 (0.17) & 0.292 (0.119) \\
$\tau^2 = 0$, $\rho_H$  & 0.466 (0.057) & 0.501 (0.05) & 0.56 (0.056) & 0.56 (0.056) & 0.215 (0.136) & 0.262 (0.107) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & 0.394 (0.06) & 0.466 (0.055) & 0.55 (0.073) & 0.55 (0.073) & 0.128 (0.122) & 0.231 (0.109) \\
$\tau^2 \ne 0$, $\rho_H$  & 0.41 (0.06) & 0.482 (0.055) & 0.566 (0.073) & 0.566 (0.073) & 0.151 (0.123) & 0.225 (0.107) \\
\hline
\end{tabular}
% \caption{Using restricted SNPs.}
% \label{tab:ldl-2}
% \end{subtable}\vspace{6pt}
\caption{LDL-c}
\label{tab:ldl}
\end{table}

%% HDL
\begin{table} \footnotesize \centering
% \begin{subtable}[t]{\textwidth} \centering
% \begin{tabular}{lcccccc}
% \hline
%  & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
% \hline
% \# SNPs  & \multicolumn{2}{c}{1130} & \multicolumn{2}{c}{42} & \multicolumn{2}{c}{1088} \\
% $p_1$  & \multicolumn{2}{c}{0.9} & \multicolumn{2}{c}{0.79} & \multicolumn{2}{c}{0.84} \\
% $\sigma_1$  & \multicolumn{2}{c}{0.82} & \multicolumn{2}{c}{8.36} & \multicolumn{2}{c}{0.63} \\
% $\sigma_2$  & \multicolumn{2}{c}{6.9} & \multicolumn{2}{c}{15.48} & \multicolumn{2}{c}{2.67} \\
% Egger  & \multicolumn{2}{c}{-0.105 (0.038)} & \multicolumn{2}{c}{0.09 (0.095)} & \multicolumn{2}{c}{-0.184 (0.074)} \\
% Wtd.\ Med.  & \multicolumn{2}{c}{0 (0.067)} & \multicolumn{2}{c}{0.005 (0.067)} & \multicolumn{2}{c}{-0.074 (0.077)} \\
% \hline %  &  &  &  &  &  &  \\
%   & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
% $\tau^2 = 0$, $\rho_{l_2}$  & -0.103 (0.034) & -0.103 (0.033) & -0.086 (0.036) & -0.086 (0.036) & -0.158 (0.089) & -0.191 (0.078) \\
% $\tau^2 = 0$, $\rho_H$  & -0.113 (0.035) & -0.106 (0.033) & -0.091 (0.036) & -0.09 (0.036) & -0.154 (0.086) & -0.174 (0.078) \\
% $\tau^2 \ne 0$, $\rho_{l_2}$  & -0.103 (0.038) & -0.106 (0.036) & -0.12 (0.058) & -0.119 (0.058) & -0.13 (0.086) & -0.167 (0.079) \\
% $\tau^2 \ne 0$, $\rho_H$  & -0.106 (0.038) & -0.106 (0.037) & -0.137 (0.062) & -0.137 (0.062) & -0.112 (0.087) & -0.136 (0.081) \\
% \hline
% \end{tabular}
% \caption{Using unrestricted SNPs.}
% \label{tab:hdl-1}
% \end{subtable}\vspace{6pt}

% \begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1122} & \multicolumn{2}{c}{23} & \multicolumn{2}{c}{1099} \\
$p_1$  & \multicolumn{2}{c}{0.91} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.83} \\
$\sigma_1$  & \multicolumn{2}{c}{0.73} & \multicolumn{2}{c}{7.85} & \multicolumn{2}{c}{0.58} \\
$\sigma_2$  & \multicolumn{2}{c}{4.57} & \multicolumn{2}{c}{7.85} & \multicolumn{2}{c}{2.17} \\
Egger  & \multicolumn{2}{c}{-0.117 (0.055)} & \multicolumn{2}{c}{-0.018 (0.196)} & \multicolumn{2}{c}{-0.132 (0.08)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{-0.118 (0.078)} & \multicolumn{2}{c}{-0.108 (0.099)} & \multicolumn{2}{c}{-0.135 (0.086)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & -0.164 (0.059) & -0.174 (0.054) & -0.109 (0.063) & -0.109 (0.063) & -0.241 (0.112) & -0.293 (0.101) \\
$\tau^2 = 0$, $\rho_H$  & -0.21 (0.059) & -0.223 (0.055) & -0.147 (0.064) & -0.147 (0.064) & -0.28 (0.11) & -0.328 (0.101) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & -0.146 (0.06) & -0.16 (0.056) & -0.103 (0.085) & -0.103 (0.085) & -0.199 (0.106) & -0.252 (0.1) \\
$\tau^2 \ne 0$, $\rho_H$  & -0.186 (0.061) & -0.204 (0.057) & -0.126 (0.088) & -0.126 (0.088) & -0.231 (0.109) & -0.283 (0.102) \\
\hline
\end{tabular}
% \caption{Using restricted SNPs.}
% \label{tab:hdl-2}
% \end{subtable}\vspace{6pt}
\caption{HDL-c}
\label{tab:hdl}
\end{table}

%% TG
\begin{table} \footnotesize \centering
% \begin{subtable}[t]{\textwidth} \centering
% \begin{tabular}{lcccccc}
% \hline
%  & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
% \hline
% \# SNPs  & \multicolumn{2}{c}{1140} & \multicolumn{2}{c}{26} & \multicolumn{2}{c}{1114} \\
% $p_1$  & \multicolumn{2}{c}{0.95} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.79} \\
% $\sigma_1$  & \multicolumn{2}{c}{0.71} & \multicolumn{2}{c}{11.08} & \multicolumn{2}{c}{0.34} \\
% $\sigma_2$  & \multicolumn{2}{c}{7.82} & \multicolumn{2}{c}{11.08} & \multicolumn{2}{c}{1.85} \\
% Egger  & \multicolumn{2}{c}{0.166 (0.046)} & \multicolumn{2}{c}{0.095 (0.1)} & \multicolumn{2}{c}{0.244 (0.095)} \\
% Wtd.\ Med.  & \multicolumn{2}{c}{0.151 (0.06)} & \multicolumn{2}{c}{0.16 (0.058)} & \multicolumn{2}{c}{0.15 (0.092)} \\
% \hline %  &  &  &  &  &  &  \\
%   & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
% $\tau^2 = 0$, $\rho_{l_2}$  & 0.252 (0.047) & 0.201 (0.042) & 0.153 (0.042) & 0.153 (0.042) & 0.84 (0.208) & 0.711 (0.19) \\
% $\tau^2 = 0$, $\rho_H$  & 0.256 (0.046) & 0.219 (0.042) & 0.179 (0.043) & 0.179 (0.043) & 0.759 (0.173) & 0.688 (0.154) \\
% $\tau^2 \ne 0$, $\rho_{l_2}$  & 0.224 (0.049) & 0.187 (0.046) & 0.154 (0.058) & 0.154 (0.058) & 0.529 (0.155) & 0.48 (0.147) \\
% $\tau^2 \ne 0$, $\rho_H$  & 0.237 (0.049) & 0.209 (0.046) & 0.178 (0.055) & 0.178 (0.055) & 0.494 (0.156) & 0.485 (0.144) \\
% \hline
% \end{tabular}
% \caption{Using unrestricted SNPs.}
% \label{tab:tg-1}
% \end{subtable}\vspace{6pt}
% \begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1114} & \multicolumn{2}{c}{8} & \multicolumn{2}{c}{1106} \\
$p_1$  & \multicolumn{2}{c}{0.98} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.97} \\
$\sigma_1$  & \multicolumn{2}{c}{0.58} & \multicolumn{2}{c}{10.25} & \multicolumn{2}{c}{0.52} \\
$\sigma_2$  & \multicolumn{2}{c}{7.04} & \multicolumn{2}{c}{10.25} & \multicolumn{2}{c}{2.48} \\
Egger  & \multicolumn{2}{c}{0.04 (0.075)} & \multicolumn{2}{c}{-0.3 (0.354)} & \multicolumn{2}{c}{0.198 (0.105)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.071 (0.109)} & \multicolumn{2}{c}{0.007 (0.108)} & \multicolumn{2}{c}{0.079 (0.103)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & 0.19 (0.134) & -0.028 (0.09) & -0.104 (0.085) & -0.104 (0.085) & 1.688 (0.647) & NA (NA) \\
$\tau^2 = 0$, $\rho_H$  & 0.246 (0.111) & 0.022 (0.085) & -0.034 (0.087) & -0.034 (0.087) & 1.535 (0.372) & 0.975 (0.289) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & 0.126 (0.111) & -0.045 (0.094) & -0.177 (0.145) & -0.177 (0.145) & 0.525 (0.235) & 0.357 (0.22) \\
$\tau^2 \ne 0$, $\rho_H$  & 0.165 (0.109) & 0.009 (0.092) & NA (NA) & NA (NA) & 0.574 (0.238) & 0.428 (0.214) \\
\hline
\end{tabular}
% \caption{Using restricted SNPs.}
% \label{tab:tg-2}
% \end{subtable}\vspace{6pt}
\caption{TG}
\label{tab:tg}
\end{table}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> result3.tex <==
%%% Validation

%% LDL
\begin{table} \scriptsize \centering
\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1141} & \multicolumn{2}{c}{37} & \multicolumn{2}{c}{1104} \\
$p_1$  & \multicolumn{2}{c}{0.92} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.88} \\
$\sigma_1$  & \multicolumn{2}{c}{0.54} & \multicolumn{2}{c}{0.11} & \multicolumn{2}{c}{0.39} \\
$\sigma_2$  & \multicolumn{2}{c}{7.26} & \multicolumn{2}{c}{10.88} & \multicolumn{2}{c}{2.36} \\
Egger  & \multicolumn{2}{c}{0.0111 (0.0011)} & \multicolumn{2}{c}{0.0128 (0.0023)} & \multicolumn{2}{c}{0.0055 (0.0025)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.0124 (0.0016)} & \multicolumn{2}{c}{0.0129 (0.0015)} & \multicolumn{2}{c}{0.0049 (0.0031)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & 0.0123 (0.0011) & 0.0123 (0.001) & 0.012 (0.001) & 0.012 (0.001) & 0.0149 (0.0048) & 0.0143 (0.0038) \\
$\tau^2 = 0$, $\rho_H$  & 0.0128 (0.0011) & 0.0127 (0.001) & 0.0126 (0.0011) & 0.0126 (0.0011) & 0.0145 (0.0044) & 0.014 (0.0036) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & 0.0115 (0.0012) & 0.0118 (0.0011) & 0.0116 (0.0013) & 0.0116 (0.0013) & 0.0103 (0.0039) & 0.0113 (0.0035) \\
$\tau^2 \ne 0$, $\rho_H$  & 0.0121 (0.0012) & 0.0123 (0.0011) & NA (NA) & 0.0126 (0.0011) & 0.0098 (0.004) & 0.011 (0.0036) \\
\hline
\end{tabular}
\caption{Using unrestricted SNPs.}
\end{subtable}\vspace{6pt}
\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1110} & \multicolumn{2}{c}{27} & \multicolumn{2}{c}{1083} \\
$p_1$  & \multicolumn{2}{c}{0.92} & \multicolumn{2}{c}{0.85} & \multicolumn{2}{c}{0.88} \\
$\sigma_1$  & \multicolumn{2}{c}{0.46} & \multicolumn{2}{c}{7.65} & \multicolumn{2}{c}{0.32} \\
$\sigma_2$  & \multicolumn{2}{c}{5.66} & \multicolumn{2}{c}{15.61} & \multicolumn{2}{c}{2.47} \\
Egger  & \multicolumn{2}{c}{0.0095 (0.0014)} & \multicolumn{2}{c}{0.0109 (0.0026)} & \multicolumn{2}{c}{0.0062 (0.0024)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.0108 (0.002)} & \multicolumn{2}{c}{0.0122 (0.0021)} & \multicolumn{2}{c}{0.0073 (0.0029)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & 0.0116 (0.0015) & 0.0116 (0.0014) & 0.0107 (0.0015) & 0.0107 (0.0015) & 0.0146 (0.0043) & 0.0143 (0.0036) \\
$\tau^2 = 0$, $\rho_H$  & 0.0116 (0.0015) & 0.0115 (0.0014) & 0.0108 (0.0015) & 0.0108 (0.0015) & 0.0144 (0.004) & 0.0144 (0.0034) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & 0.0109 (0.0015) & 0.0112 (0.0014) & 0.0106 (0.0015) & 0.0106 (0.0015) & 0.0115 (0.0038) & 0.0124 (0.0034) \\
$\tau^2 \ne 0$, $\rho_H$  & 0.011 (0.0016) & 0.0112 (0.0015) & 0.0108 (0.0015) & 0.0108 (0.0015) & 0.0118 (0.0039) & 0.0127 (0.0034) \\
\hline
\end{tabular}
\caption{Using restricted SNPs.}
\end{subtable}\vspace{6pt}
\caption{LDL-c}
\end{table}

%% HDL
\begin{table} \scriptsize \centering
\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1071} & \multicolumn{2}{c}{39} & \multicolumn{2}{c}{1032} \\
$p_1$  & \multicolumn{2}{c}{0.88} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.85} \\
$\sigma_1$  & \multicolumn{2}{c}{0.77} & \multicolumn{2}{c}{9.15} & \multicolumn{2}{c}{0.65} \\
$\sigma_2$  & \multicolumn{2}{c}{5.9} & \multicolumn{2}{c}{9.15} & \multicolumn{2}{c}{2.82} \\
Egger  & \multicolumn{2}{c}{-0.0056 (0.0014)} & \multicolumn{2}{c}{0.0098 (0.0044)} & \multicolumn{2}{c}{-0.0121 (0.0023)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{-0.0041 (0.0019)} & \multicolumn{2}{c}{-6e-04 (0.0026)} & \multicolumn{2}{c}{-0.0071 (0.0025)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & -0.0073 (0.0013) & -0.0065 (0.0012) & -0.0039 (0.0014) & -0.0039 (0.0014) & -0.0144 (0.0027) & -0.0145 (0.0025) \\
$\tau^2 = 0$, $\rho_H$  & -0.01 (0.0013) & -0.0091 (0.0012) & -0.0075 (0.0014) & -0.0075 (0.0014) & -0.0127 (0.0026) & -0.0121 (0.0024) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & -0.0069 (0.0014) & -0.0063 (0.0013) & -0.0041 (0.0027) & -0.0041 (0.0027) & -0.0137 (0.0027) & -0.0139 (0.0025) \\
$\tau^2 \ne 0$, $\rho_H$  & -0.0095 (0.0013) & -0.0087 (0.0013) & -0.0045 (0.0028) & -0.0045 (0.0028) & -0.0122 (0.0027) & -0.0118 (0.0025) \\
\hline
\end{tabular}
\caption{Using unrestricted SNPs.}
\end{subtable}\vspace{6pt}
\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1071} & \multicolumn{2}{c}{19} & \multicolumn{2}{c}{1052} \\
$p_1$  & \multicolumn{2}{c}{0.89} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.8} \\
$\sigma_1$  & \multicolumn{2}{c}{0.73} & \multicolumn{2}{c}{8.04} & \multicolumn{2}{c}{0.54} \\
$\sigma_2$  & \multicolumn{2}{c}{4.31} & \multicolumn{2}{c}{8.04} & \multicolumn{2}{c}{2.31} \\
Egger  & \multicolumn{2}{c}{-0.0059 (0.0017)} & \multicolumn{2}{c}{0.0158 (0.0058)} & \multicolumn{2}{c}{-0.0132 (0.0023)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{-0.0052 (0.0023)} & \multicolumn{2}{c}{0.0037 (0.0036)} & \multicolumn{2}{c}{-0.0083 (0.0026)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & -0.0074 (0.0019) & -0.0062 (0.0017) & 0.0014 (0.0022) & 0.0014 (0.0022) & -0.0154 (0.0029) & -0.0161 (0.0027) \\
$\tau^2 = 0$, $\rho_H$  & -0.0096 (0.0019) & -0.0088 (0.0017) & 3e-04 (0.0022) & 3e-04 (0.0022) & -0.0149 (0.003) & -0.0156 (0.0027) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & -0.0069 (0.0019) & -0.0058 (0.0018) & 0.0021 (0.003) & 0.0021 (0.003) & -0.0147 (0.0029) & -0.0155 (0.0027) \\
$\tau^2 \ne 0$, $\rho_H$  & -0.009 (0.0019) & -0.0082 (0.0018) & 0.0015 (0.0032) & 0.0015 (0.0032) & -0.014 (0.003) & -0.0149 (0.0028) \\
\hline
\end{tabular}
\caption{Using restricted SNPs.}
\end{subtable}\vspace{6pt}
\caption{HDL-c}
\end{table}

%% TG
\begin{table} \scriptsize \centering
\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1125} & \multicolumn{2}{c}{27} & \multicolumn{2}{c}{1098} \\
$p_1$  & \multicolumn{2}{c}{0.95} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.84} \\
$\sigma_1$  & \multicolumn{2}{c}{0.63} & \multicolumn{2}{c}{11.68} & \multicolumn{2}{c}{0.33} \\
$\sigma_2$  & \multicolumn{2}{c}{8.25} & \multicolumn{2}{c}{11.68} & \multicolumn{2}{c}{1.98} \\
Egger  & \multicolumn{2}{c}{0.0089 (0.0013)} & \multicolumn{2}{c}{0.0037 (0.0034)} & \multicolumn{2}{c}{0.0136 (0.0028)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.0079 (0.0019)} & \multicolumn{2}{c}{0.008 (0.0018)} & \multicolumn{2}{c}{0.0091 (0.003)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & 0.0126 (0.0013) & 0.0106 (0.0013) & 0.0084 (0.0013) & 0.0084 (0.0013) & 0.0316 (0.0046) & 0.0289 (0.0042) \\
$\tau^2 = 0$, $\rho_H$  & 0.0137 (0.0014) & 0.0109 (0.0013) & 0.008 (0.0013) & 0.008 (0.0013) & 0.0297 (0.0045) & 0.0253 (0.0041) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & 0.0119 (0.0014) & 0.0102 (0.0013) & 0.0077 (0.002) & 0.0077 (0.002) & 0.0292 (0.0047) & 0.0273 (0.0043) \\
$\tau^2 \ne 0$, $\rho_H$  & 0.0128 (0.0014) & 0.0105 (0.0013) & 0.0076 (0.002) & 0.0076 (0.002) & 0.0279 (0.0047) & 0.0244 (0.0042) \\
\hline
\end{tabular}
\caption{Using unrestricted SNPs.}
\end{subtable}\vspace{6pt}
\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1112} & \multicolumn{2}{c}{7} & \multicolumn{2}{c}{1105} \\
$p_1$  & \multicolumn{2}{c}{0.98} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.99} \\
$\sigma_1$  & \multicolumn{2}{c}{0.57} & \multicolumn{2}{c}{9.65} & \multicolumn{2}{c}{0.59} \\
$\sigma_2$  & \multicolumn{2}{c}{7.25} & \multicolumn{2}{c}{9.65} & \multicolumn{2}{c}{6.89} \\
Egger  & \multicolumn{2}{c}{0.0079 (0.002)} & \multicolumn{2}{c}{-0.0015 (0.0092)} & \multicolumn{2}{c}{0.0106 (0.0024)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.0062 (0.0034)} & \multicolumn{2}{c}{0.0061 (0.0037)} & \multicolumn{2}{c}{0.0158 (0.0036)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\rho_{l_2}$  & 0.014 (0.0027) & 0.0098 (0.0023) & 0.0031 (0.0031) & 0.0031 (0.0031) & 0.0218 (0.0041) & 0.0172 (0.0033) \\
$\tau^2 = 0$, $\rho_H$  & 0.0166 (0.0027) & 0.011 (0.0023) & 0.0038 (0.0031) & 0.0038 (0.0031) & 0.0225 (0.0041) & 0.0172 (0.0034) \\
$\tau^2 \ne 0$, $\rho_{l_2}$  & 0.0135 (0.0027) & 0.0096 (0.0023) & 0.0026 (0.0037) & 0.0026 (0.0037) & 0.021 (0.0041) & 0.0168 (0.0033) \\
$\tau^2 \ne 0$, $\rho_H$  & 0.0159 (0.0028) & 0.0108 (0.0024) & NA (NA) & NA (NA) & 0.0218 (0.0042) & 0.017 (0.0034) \\
\hline
\end{tabular}
\caption{Using restricted SNPs.}
\end{subtable}\vspace{6pt}
\caption{TG}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> result4.tex <==
%% primary
\begin{table} \footnotesize \centering
\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1120} & \multicolumn{2}{c}{27} & \multicolumn{2}{c}{1093} \\
$p_1$  & \multicolumn{2}{c}{0.92} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.91} \\
$\sigma_1$  & \multicolumn{2}{c}{0.52} & \multicolumn{2}{c}{7.96} & \multicolumn{2}{c}{0.46} \\
$\sigma_2$  & \multicolumn{2}{c}{5.01} & \multicolumn{2}{c}{7.96} & \multicolumn{2}{c}{2.61} \\
MR-Egger  & \multicolumn{2}{c}{0.368 (0.053)} & \multicolumn{2}{c}{0.892 (0.134)} & \multicolumn{2}{c}{0.057 (0.08)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.534 (0.071)} & \multicolumn{2}{c}{0.552 (0.075)} & \multicolumn{2}{c}{0.166 (0.094)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\psi_I$  & 0.448 (0.06) & 0.484 (0.05) & 0.528 (0.055) & 0.528 (0.055) & 0.204 (0.17) & 0.292 (0.119) \\
$\tau^2 = 0$, $\psi_H$  & 0.466 (0.057) & 0.501 (0.05) & 0.56 (0.056) & 0.56 (0.056) & 0.215 (0.136) & 0.262 (0.107) \\
$\tau^2 \ne 0$, $\psi_I$  & 0.394 (0.06) & 0.466 (0.055) & 0.55 (0.073) & 0.55 (0.073) & 0.128 (0.122) & 0.231 (0.109) \\
$\tau^2 \ne 0$, $\psi_H$  & 0.41 (0.06) & \textbf{0.482 (0.055)} & 0.566 (0.073) & 0.566 (0.073) & 0.151 (0.123) & 0.225 (0.107) \\
\hline
\end{tabular}
\caption{Low-density lipoprotein cholesterol (LDL-c).}
\label{tab:ldl-1}
\end{subtable}\vspace{6pt}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1122} & \multicolumn{2}{c}{23} & \multicolumn{2}{c}{1099} \\
$p_1$  & \multicolumn{2}{c}{0.91} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.83} \\
$\sigma_1$  & \multicolumn{2}{c}{0.73} & \multicolumn{2}{c}{7.85} & \multicolumn{2}{c}{0.58} \\
$\sigma_2$  & \multicolumn{2}{c}{4.57} & \multicolumn{2}{c}{7.85} & \multicolumn{2}{c}{2.17} \\
MR-Egger  & \multicolumn{2}{c}{-0.117 (0.055)} & \multicolumn{2}{c}{-0.018 (0.196)} & \multicolumn{2}{c}{-0.132 (0.08)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{-0.118 (0.078)} & \multicolumn{2}{c}{-0.108 (0.099)} & \multicolumn{2}{c}{-0.135 (0.086)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\psi_I$  & -0.164 (0.059) & -0.174 (0.054) & -0.109 (0.063) & -0.109 (0.063) & -0.241 (0.112) & -0.293 (0.101) \\
$\tau^2 = 0$, $\psi_H$  & -0.21 (0.059) & -0.223 (0.055) & -0.147 (0.064) & -0.147 (0.064) & -0.28 (0.11) & -0.328 (0.101) \\
$\tau^2 \ne 0$, $\psi_I$  & -0.146 (0.06) & -0.16 (0.056) & -0.103 (0.085) & -0.103 (0.085) & -0.199 (0.106) & -0.252 (0.1) \\
$\tau^2 \ne 0$, $\psi_H$  & -0.186 (0.061) & \textbf{-0.204 (0.057)} & -0.126 (0.088) & -0.126 (0.088) & -0.231 (0.109) & -0.283 (0.102) \\
\hline
\end{tabular}
\caption{High-density lipoprotein cholesterol (HDL-c).}
\label{tab:hdl-1}
\end{subtable}

\vspace{6pt}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1114} & \multicolumn{2}{c}{8} & \multicolumn{2}{c}{1106} \\
$p_1$  & \multicolumn{2}{c}{0.98} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.97} \\
$\sigma_1$  & \multicolumn{2}{c}{0.58} & \multicolumn{2}{c}{10.25} & \multicolumn{2}{c}{0.52} \\
$\sigma_2$  & \multicolumn{2}{c}{7.04} & \multicolumn{2}{c}{10.25} & \multicolumn{2}{c}{2.48} \\
MR-Egger  & \multicolumn{2}{c}{0.04 (0.075)} & \multicolumn{2}{c}{-0.3 (0.354)} & \multicolumn{2}{c}{0.198 (0.105)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.071 (0.109)} & \multicolumn{2}{c}{0.007 (0.108)} & \multicolumn{2}{c}{0.079 (0.103)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\psi_I$  & 0.19 (0.134) & -0.028 (0.09) & -0.104 (0.085) & -0.104 (0.085) & 1.688 (0.647) & NA (NA) \\
$\tau^2 = 0$, $\psi_H$  & 0.246 (0.111) & 0.022 (0.085) & -0.034 (0.087) & -0.034 (0.087) & 1.535 (0.372) & 0.975 (0.289) \\
$\tau^2 \ne 0$, $\psi_I$  & 0.126 (0.111) & -0.045 (0.094) & -0.177 (0.145) & -0.177 (0.145) & 0.525 (0.235) & 0.357 (0.22) \\
$\tau^2 \ne 0$, $\psi_H$  & 0.165 (0.109) & \textbf{0.009 (0.092)} & NA (NA) & NA (NA) & 0.574 (0.238) & 0.428 (0.214) \\
\hline
\end{tabular}
\caption{Triglycerides (TG).}
\label{tab:tg-1}
\end{subtable}

\caption{Primary analysis for coronary artery disease (CAD). Bolded
  cells correspond to the recommended analysis: $\tau^2 \ne 0$,
  robust Huber score function $\rho_H$, and empirical partially Bayes shrinkage.}
\label{tab:primary}
\end{table}

%% HDL
\begin{table} \footnotesize \centering
% \begin{subtable}[t]{\textwidth} \centering
% \begin{tabular}{l|cccccc}
% \hline
%  & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
% \hline
% \# SNPs  & \multicolumn{2}{c}{1130} & \multicolumn{2}{c}{42} & \multicolumn{2}{c}{1088} \\
% $p_1$  & \multicolumn{2}{c}{0.9} & \multicolumn{2}{c}{0.79} & \multicolumn{2}{c}{0.84} \\
% $\sigma_1$  & \multicolumn{2}{c}{0.82} & \multicolumn{2}{c}{8.36} & \multicolumn{2}{c}{0.63} \\
% $\sigma_2$  & \multicolumn{2}{c}{6.9} & \multicolumn{2}{c}{15.48} & \multicolumn{2}{c}{2.67} \\
% MR-Egger  & \multicolumn{2}{c}{-0.105 (0.038)} & \multicolumn{2}{c}{0.09 (0.095)} & \multicolumn{2}{c}{-0.184 (0.074)} \\
% Wtd.\ Med.  & \multicolumn{2}{c}{0 (0.067)} & \multicolumn{2}{c}{0.005 (0.067)} & \multicolumn{2}{c}{-0.074 (0.077)} \\
% \hline %  &  &  &  &  &  &  \\
%   & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
% $\tau^2 = 0$, $\psi_I$  & -0.103 (0.034) & -0.103 (0.033) & -0.086 (0.036) & -0.086 (0.036) & -0.158 (0.089) & -0.191 (0.078) \\
% $\tau^2 = 0$, $\psi_H$  & -0.113 (0.035) & -0.106 (0.033) & -0.091 (0.036) & -0.09 (0.036) & -0.154 (0.086) & -0.174 (0.078) \\
% $\tau^2 \ne 0$, $\psi_I$  & -0.103 (0.038) & -0.106 (0.036) & -0.12 (0.058) & -0.119 (0.058) & -0.13 (0.086) & -0.167 (0.079) \\
% $\tau^2 \ne 0$, $\psi_H$  & -0.106 (0.038) & -0.106 (0.037) & -0.137 (0.062) & -0.137 (0.062) & -0.112 (0.087) & -0.136 (0.081) \\
% \hline
% \end{tabular}
% \caption{Using unrestricted SNPs.}
% \label{tab:hdl-1}
% \end{subtable}\vspace{6pt}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1110} & \multicolumn{2}{c}{27} & \multicolumn{2}{c}{1083} \\
$p_1$  & \multicolumn{2}{c}{0.92} & \multicolumn{2}{c}{0.85} & \multicolumn{2}{c}{0.88} \\
$\sigma_1$  & \multicolumn{2}{c}{0.46} & \multicolumn{2}{c}{7.65} & \multicolumn{2}{c}{0.32} \\
$\sigma_2$  & \multicolumn{2}{c}{5.66} & \multicolumn{2}{c}{15.61} & \multicolumn{2}{c}{2.47} \\
MR-Egger  & \multicolumn{2}{c}{0.0095 (0.0014)} & \multicolumn{2}{c}{0.0109 (0.0026)} & \multicolumn{2}{c}{0.0062 (0.0024)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.0108 (0.002)} & \multicolumn{2}{c}{0.0122 (0.0021)} & \multicolumn{2}{c}{0.0073 (0.0029)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\psi_I$  & 0.0116 (0.0015) & 0.0116 (0.0014) & 0.0107 (0.0015) & 0.0107 (0.0015) & 0.0146 (0.0043) & 0.0143 (0.0036) \\
$\tau^2 = 0$, $\psi_H$  & 0.0116 (0.0015) & 0.0115 (0.0014) & 0.0108 (0.0015) & 0.0108 (0.0015) & 0.0144 (0.004) & 0.0144 (0.0034) \\
$\tau^2 \ne 0$, $\psi_I$  & 0.0109 (0.0015) & 0.0112 (0.0014) & 0.0106 (0.0015) & 0.0106 (0.0015) & 0.0115 (0.0038) & 0.0124 (0.0034) \\
$\tau^2 \ne 0$, $\psi_H$  & 0.011 (0.0016) & \textbf{0.0112 (0.0015)} & 0.0108 (0.0015) & 0.0108 (0.0015) & 0.0118 (0.0039) & 0.0127 (0.0034) \\
\hline
\end{tabular}
\caption{Low-density lipoprotein cholesterol (LDL-c).}
\label{tab:ldl-2}
\end{subtable}

\vspace{6pt}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1071} & \multicolumn{2}{c}{19} & \multicolumn{2}{c}{1052} \\
$p_1$  & \multicolumn{2}{c}{0.89} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.8} \\
$\sigma_1$  & \multicolumn{2}{c}{0.73} & \multicolumn{2}{c}{8.04} & \multicolumn{2}{c}{0.54} \\
$\sigma_2$  & \multicolumn{2}{c}{4.31} & \multicolumn{2}{c}{8.04} & \multicolumn{2}{c}{2.31} \\
MR-Egger  & \multicolumn{2}{c}{-0.0059 (0.0017)} & \multicolumn{2}{c}{0.0158 (0.0058)} & \multicolumn{2}{c}{-0.0132 (0.0023)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{-0.0052 (0.0023)} & \multicolumn{2}{c}{0.0037 (0.0036)} & \multicolumn{2}{c}{-0.0083 (0.0026)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\psi_I$  & -0.0074 (0.0019) & -0.0062 (0.0017) & 0.0014 (0.0022) & 0.0014 (0.0022) & -0.0154 (0.0029) & -0.0161 (0.0027) \\
$\tau^2 = 0$, $\psi_H$  & -0.0096 (0.0019) & -0.0088 (0.0017) & 0.0003 (0.0022) & 0.0003 (0.0022) & -0.0149 (0.003) & -0.0156 (0.0027) \\
$\tau^2 \ne 0$, $\psi_I$  & -0.0069 (0.0019) & -0.0058 (0.0018) & 0.0021 (0.003) & 0.0021 (0.003) & -0.0147 (0.0029) & -0.0155 (0.0027) \\
$\tau^2 \ne 0$, $\psi_H$  & -0.009 (0.0019) & \textbf{-0.0082 (0.0018)} & 0.0015 (0.0032) & 0.0015 (0.0032) & -0.014 (0.003) & -0.0149 (0.0028) \\
\hline
\end{tabular}
\caption{High-density lipoprotein cholesterol (HDL-c).}
\label{tab:hdl-2}
\end{subtable}

\vspace{6pt}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1112} & \multicolumn{2}{c}{7} & \multicolumn{2}{c}{1105} \\
$p_1$  & \multicolumn{2}{c}{0.98} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.99} \\
$\sigma_1$  & \multicolumn{2}{c}{0.57} & \multicolumn{2}{c}{9.65} & \multicolumn{2}{c}{0.59} \\
$\sigma_2$  & \multicolumn{2}{c}{7.25} & \multicolumn{2}{c}{9.65} & \multicolumn{2}{c}{6.89} \\
MR-Egger  & \multicolumn{2}{c}{0.0079 (0.002)} & \multicolumn{2}{c}{-0.0015 (0.0092)} & \multicolumn{2}{c}{0.0106 (0.0024)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.0062 (0.0034)} & \multicolumn{2}{c}{0.0061 (0.0037)} & \multicolumn{2}{c}{0.0158 (0.0036)} \\
\hline %  &  &  &  &  &  &  \\
  & Profile & Shrinkage & Profile & Shrinkage & Profile & \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\psi_I$  & 0.014 (0.0027) & 0.0098 (0.0023) & 0.0031 (0.0031) & 0.0031 (0.0031) & 0.0218 (0.0041) & 0.0172 (0.0033) \\
$\tau^2 = 0$, $\psi_H$  & 0.0166 (0.0027) & 0.011 (0.0023) & 0.0038 (0.0031) & 0.0038 (0.0031) & 0.0225 (0.0041) & 0.0172 (0.0034) \\
$\tau^2 \ne 0$, $\psi_I$  & 0.0135 (0.0027) & 0.0096 (0.0023) & 0.0026 (0.0037) & 0.0026 (0.0037) & 0.021 (0.0041) & 0.0168 (0.0033) \\
$\tau^2 \ne 0$, $\psi_H$  & 0.0159 (0.0028) & \textbf{0.0108 (0.0024)} & NA (NA) & NA (NA) & 0.0218 (0.0042) & 0.017 (0.0034) \\
\hline
\end{tabular}
\caption{Triglycerides (TG).}
\label{tab:tg-2}
\end{subtable}

\caption{Secondary analysis for self-reported myocardial infarction. Bolded
  cells correspond to the recommended analysis: $\tau^2 \ne 0$,
  robust Huber score function $\rho_H$, and empirical partially Bayes
  shrinkage.}
\label{tab:secondary}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> result_secondary.tex <==
%% HDL
\begin{table} \footnotesize \centering \renewcommand\thetable{B1}
% \begin{subtable}[t]{\textwidth} \centering
% \begin{tabular}{l|cccccc}
% \hline
%  & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
% \hline
% \# SNPs  & \multicolumn{2}{c}{1130} & \multicolumn{2}{c}{42} & \multicolumn{2}{c}{1088} \\
% $p_1$  & \multicolumn{2}{c}{0.9} & \multicolumn{2}{c}{0.79} & \multicolumn{2}{c}{0.84} \\
% $\sigma_1$  & \multicolumn{2}{c}{0.82} & \multicolumn{2}{c}{8.36} & \multicolumn{2}{c}{0.63} \\
% $\sigma_2$  & \multicolumn{2}{c}{6.9} & \multicolumn{2}{c}{15.48} & \multicolumn{2}{c}{2.67} \\
% MR-Egger  & \multicolumn{2}{c}{-0.105 (0.038)} & \multicolumn{2}{c}{0.09 (0.095)} & \multicolumn{2}{c}{-0.184 (0.074)} \\
% Wtd.\ Med.  & \multicolumn{2}{c}{0 (0.067)} & \multicolumn{2}{c}{0.005 (0.067)} & \multicolumn{2}{c}{-0.074 (0.077)} \\
% \hline %  &  &  &  &  &  &  \\
%   & MLE & Shrinkage & MLE & Shrinkage & MLE & \multicolumn{1}{c}{Shrinkage} \\
% $\tau^2 = 0$, $\psi_I$  & -0.103 (0.034) & -0.103 (0.033) & -0.086 (0.036) & -0.086 (0.036) & -0.158 (0.089) & -0.191 (0.078) \\
% $\tau^2 = 0$, $\psi_H$  & -0.113 (0.035) & -0.106 (0.033) & -0.091 (0.036) & -0.09 (0.036) & -0.154 (0.086) & -0.174 (0.078) \\
% $\tau^2 \ne 0$, $\psi_I$  & -0.103 (0.038) & -0.106 (0.036) & -0.12 (0.058) & -0.119 (0.058) & -0.13 (0.086) & -0.167 (0.079) \\
% $\tau^2 \ne 0$, $\psi_H$  & -0.106 (0.038) & -0.106 (0.037) & -0.137 (0.062) & -0.137 (0.062) & -0.112 (0.087) & -0.136 (0.081) \\
% \hline
% \end{tabular}
% \caption{Using unrestricted SNPs.}
% \label{tab:hdl-1}
% \end{subtable}\vspace{6pt}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1110} & \multicolumn{2}{c}{27} & \multicolumn{2}{c}{1083} \\
$p_1$  & \multicolumn{2}{c}{0.92} & \multicolumn{2}{c}{0.85} & \multicolumn{2}{c}{0.88} \\
$\sigma_1$  & \multicolumn{2}{c}{0.46} & \multicolumn{2}{c}{7.65} & \multicolumn{2}{c}{0.32} \\
$\sigma_2$  & \multicolumn{2}{c}{5.66} & \multicolumn{2}{c}{15.61} & \multicolumn{2}{c}{2.47} \\
MR-Egger  & \multicolumn{2}{c}{0.355 (0.045)} & \multicolumn{2}{c}{0.399 (0.08)} & \multicolumn{2}{c}{0.245 (0.086)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.396 (0.06)} & \multicolumn{2}{c}{0.44 (0.062)} & \multicolumn{2}{c}{0.283 (0.102)} \\
\hline %  &  &  &  &  &  &  \\
  & MLE & Shrinkage & MLE & Shrinkage & MLE &
                                                          \multicolumn{1}{c}{Shrinkage}
  \\
  $\tau^2 = 0$, $\psi_I$  & 0.421 (0.045) & 0.42 (0.041) & 0.393 (0.045) & 0.393 (0.045) & 0.507 (0.121) & 0.5 (0.1) \\
$\tau^2 = 0$, $\psi_H$  & 0.42 (0.046) & 0.418 (0.042) & 0.396 (0.046) & 0.397 (0.046) & 0.503 (0.113) & 0.501 (0.095) \\
$\tau^2 \ne 0$, $\psi_I$  & 0.399 (0.047) & 0.408 (0.044) & 0.392 (0.048) & 0.392 (0.048) & 0.42 (0.114) & 0.443 (0.101) \\
$\tau^2 \ne 0$, $\psi_H$ & 0.402 (0.048) & \textbf{0.408 (0.044)} & 0.396 (0.046) &
                                                                   0.396 (0.046) & 0.426 (0.116) & 0.454 (0.1) \\
\hline
\end{tabular}
\caption{Low-density lipoprotein cholesterol (LDL-c).}
\label{tab:ldl-2}
\end{subtable}

\vspace{6pt}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1071} & \multicolumn{2}{c}{19} & \multicolumn{2}{c}{1052} \\
$p_1$  & \multicolumn{2}{c}{0.89} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.8} \\
$\sigma_1$  & \multicolumn{2}{c}{0.73} & \multicolumn{2}{c}{8.04} & \multicolumn{2}{c}{0.54} \\
$\sigma_2$  & \multicolumn{2}{c}{4.31} & \multicolumn{2}{c}{8.04} & \multicolumn{2}{c}{2.31} \\
MR-Egger  & \multicolumn{2}{c}{-0.304 (0.104)} & \multicolumn{2}{c}{0.541 (0.157)} & \multicolumn{2}{c}{-0.872 (0.245)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{-0.262 (0.137)} & \multicolumn{2}{c}{0.152 (0.137)} & \multicolumn{2}{c}{-0.454 (0.176)} \\
\hline %  &  &  &  &  &  &  \\
  & MLE & Shrinkage & MLE & Shrinkage & MLE &
                                                          \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\psi_I$  & -0.395 (0.122) & -0.322 (0.105) & 0.062 (0.093) & 0.062 (0.093) & -1.134 (0.414) & -1.22 (0.412) \\
$\tau^2 = 0$, $\psi_H$  & -0.555 (0.145) & -0.491 (0.126) & 0.012 (0.099) & 0.012 (0.099) & -1.064 (0.39) & -1.154 (0.389) \\
$\tau^2 \ne 0$, $\psi_I$  & -0.366 (0.12) & -0.3 (0.105) & 0.09 (0.123) & 0.09 (0.123) & -1.041 (0.375) & -1.143 (0.383) \\
$\tau^2 \ne 0$, $\psi_H$  & -0.507 (0.141) & \textbf{-0.454 (0.125)} & 0.066 (0.136) & 0.066 (0.136) & -0.96 (0.354) & -1.067 (0.362) \\
\hline
\end{tabular}
\caption{High-density lipoprotein cholesterol (HDL-c).}
\label{tab:hdl-2}
\end{subtable}

\vspace{6pt}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l|cccccc}
\hline
 & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 1)$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (0, 5 \times 10^{-8})$} & \multicolumn{2}{c}{$p_\mathrm{sel} \in (5 \times 10^{-8}, 1)$} \\
\hline
\# SNPs  & \multicolumn{2}{c}{1112} & \multicolumn{2}{c}{7} & \multicolumn{2}{c}{1105} \\
$p_1$  & \multicolumn{2}{c}{0.98} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.99} \\
$\sigma_1$  & \multicolumn{2}{c}{0.57} & \multicolumn{2}{c}{9.65} & \multicolumn{2}{c}{0.59} \\
$\sigma_2$  & \multicolumn{2}{c}{7.25} & \multicolumn{2}{c}{9.65} & \multicolumn{2}{c}{6.89} \\
MR-Egger  & \multicolumn{2}{c}{0.303 (0.066)} & \multicolumn{2}{c}{-0.069 (0.469)} & \multicolumn{2}{c}{0.392 (0.075)} \\
Wtd.\ Med.  & \multicolumn{2}{c}{0.246 (0.119)} & \multicolumn{2}{c}{0.242 (0.143)} & \multicolumn{2}{c}{0.539 (0.1)} \\
\hline %  &  &  &  &  &  &  \\
  & MLE & Shrinkage & MLE & Shrinkage & MLE &
                                                          \multicolumn{1}{c}{Shrinkage} \\
$\tau^2 = 0$, $\psi_I$  & 0.492 (0.076) & 0.366 (0.071) & 0.131 (0.121) & 0.131 (0.121) & 0.69 (0.096) & 0.576 (0.085) \\
$\tau^2 = 0$, $\psi_H$  & 0.561 (0.072) & 0.402 (0.071) & 0.155 (0.121) & 0.155 (0.121) & 0.707 (0.095) & 0.577 (0.087) \\
$\tau^2 \ne 0$, $\psi_I$  & 0.478 (0.078) & 0.359 (0.073) & 0.111 (0.149) & 0.111 (0.149) & 0.673 (0.099) & 0.568 (0.087) \\
$\tau^2 \ne 0$, $\psi_H$  & 0.544 (0.075) & \textbf{0.398 (0.072)} & NA (NA) & NA (NA) & 0.691 (0.099) & 0.573 (0.089) \\
\hline
\end{tabular}
\caption{Triglycerides (TG).}
\label{tab:tg-2}
\end{subtable}

\caption{Secondary analysis for self-reported myocardial infarction. Bolded
  cells correspond to the recommended analysis: $\tau^2 \ne 0$,
  robust Huber score function $\psi_H$, and empirical partially Bayes
  shrinkage. The numbers reported in this table can be interpreted as
  causal log odds ratios. When there were multiple roots to the
  estimating equation, the results were reported as NA (not available).}
\label{tab:secondary}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> secondary_analysis.tex <==
In our secondary analysis we use an interim release of the UK BioBank self-reported
myocardial infarction GWAS \cite{nealelabukbb}. Notice that in this
dataset the genetic associations were reported using a linear
regression model instead of the usual logistic regression model. Thus
a directly MR analysis effectively estimates the causal risk
difference. In order to compare with the results of the primary
analysis, we transformed the estimates to the log odds ratio scale
using a crude approximation formula (the overall prevelance of
self-reported myocardial infarction is 7735/337159 = 2.3\%).

The harmful effect of LDL-c and protective effect of HDL-c replicate
in the secondary analysis (\Cref{tab:ldl-2,tab:hdl-2}). However, the
analysis for TG (\Cref{tab:tg-2}) suggest its effect on CAD is
significantly positive, and the magnitude of the effect is similar to
that of LDL-c. This is drastically different from the null finding
regarding TG in our primary analysis.

\input{result_secondary}

Different from the primary analysis, the diagnostic plots of the
secondary analysis show that the heterogeneity between weak and
strong instruments is quite significant for HDL-c (\Cref{fig:hdl-2}). This
can be mostly attributed to the four strongest instruments which all have
positive standardized residuals between 2 and 4. Further investigation
is required to understand the biological mechanism of this heterogeneity.

\begin{figure} \renewcommand\thefigure{B1}
  \centering
  \begin{subfigure}[b]{\textwidth} \centering
    \includegraphics[width = 0.75\textwidth]{ldl2}
    \caption{LDL-c.}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth} \centering
    \includegraphics[width = 0.75\textwidth]{hdl2}
    \caption{HDL-c.}
    \label{fig:hdl-2}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth} \centering
    \includegraphics[width = 0.75\textwidth]{tg2}
    \caption{TG.}
  \end{subfigure}
  \caption{Diagnostic plots in the secondary analysis. If our modeling
    assumptions are satisfied, most of the standardized residuals
    ($y$-axis) should be approximately independent of the instrument
    weight ($x$-axis), checked by the scatter-plot in the left panel,
    and roughly follow the standard normal distribution, checked by
    the quantile-quantile plot in the right panel.}
  \label{fig:secondary-diagnostics}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

